Making Non-Stochastic Control (Almost) as Easy as Stochastic

Recent literature has made much progress in understanding \emph{online LQR}: a modern learning-theoretic take on the classical control problem in which a learner attempts to optimally control an unknown linear dynamical system with fully observed state, perturbed by i.i.d. Gaussian noise. It is now understood that the optimal regret on time horizon $T$ against the optimal control law scales as $\widetilde{\Theta}(\sqrt{T})$. In this paper, we show that the same regret rate (against a suitable benchmark) is attainable even in the considerably more general non-stochastic control model, where the system is driven by \emph{arbitrary adversarial} noise (Agarwal et al. 2019). In other words, \emph{stochasticity confers little benefit in online LQR}. We attain the optimal $\widetilde{\mathcal{O}}(\sqrt{T})$ regret when the dynamics are unknown to the learner, and $\mathrm{poly}(\log T)$ regret when known, provided that the cost functions are strongly convex (as in LQR). Our algorithm is based on a novel variant of online Newton step (Hazan et al. 2007), which adapts to the geometry induced by possibly adversarial disturbances, and our analysis hinges on generic "policy regret" bounds for certain structured losses in the OCO-with-memory framework (Anava et al. 2015). Moreover, our results accomodate the full generality of the non-stochastic control setting: adversarially chosen (possibly non-quadratic) costs, partial state observation, and fully adversarial process and observation noise.

==> body/algorithm.tex <==
%!TEX root = ../so_control_main.tex



==> body/body_slow.tex <==
%!TEX root = ../main.tex
\section{Rates without a condition modulus}
\subsection{Slow Rates}

From \Cref{eq:operator_norm_bound_movement}, we have that for any $t,s$,
\begin{align*}
\|\matY_s (z_{t}-z_{t-1})\|_2 &\le \eta \sqrt{\|\matY_s \Lambda_t^{-1/2}\|_{\op}^2 \| \nabla_t\|_{\Lambda_{t}^{\shortminus 1}}^2} \le \frac{\eta}{\lambda} \|\matY_s\|_{\op}\sqrt{ \| \nabla_t\|_{\Lambda_{t}^{\shortminus 1}}^2} \le \frac{\eta \radY^2}{\lambda}\sqrt{ \| \nabla_t\|_{\Lambda_{t}^{\shortminus  1}}^2},
\end{align*}
where we crudely bound $\|\matY_s \Lambda_t^{-1/2}\|_{\op}^2 = \|\matY_s \Lambda_t^{-1}\matY_s\|_{\op} \le \frac{1}{\lambda}\|\matY_s\|_{\op}^2$, as $\Lambda_t \succeq \lambda I$.  Therefore, 
\begin{align*}
	\normaltext{(movement cost)} &\le h \Leff \radG \sum_{s=1-h}^T \sum_{i=1}^{h-1} \|\matY_{s}(\matz_{s+i+1} - \matz_{s+i})\|_2 \cdot \I_{1 \le s+i \le t-1}\\
	&\le \frac{h \eta \radY^2 \Leff \radG}{\lambda}\sum_{s=1-h}^T \sum_{i=1}^{h-1} \sqrt{ \| \nabla_{s+i}\|_{\Lambda_{s+i}^{\shortminus 1}}^2} \cdot \I_{1 \le s+i \le t-1}\\
	&\le \frac{h^2 \eta \radY^2 \Leff \radG}{\lambda}\sum_{s=1}^T  \sqrt{ \| \nabla_{t}\|_{\Lambda_{t}^{\shortminus 1}}^2}.
	\end{align*}
	Now, by Cauchy-Schwartz, followed by \Cref{eq:X_move_contrib}, we bound
	\begin{align*}
	\sum_{t=1}^T  \sqrt{ \| \nabla_{t}\|_{\Lambda_{t}^{1/2}}^2} \le \sqrt{T} \cdot \frac{\eta }{2} \sum_{s=1}^T   \| \nabla_{t}\|_{\Lambda_{t}^{1/2}}^2 \le  d \Leff^2 \sqrt{T}\log\left(1 + \frac{T\radH^2}{\lambda}\right).
	\end{align*}
	Therefore,

\subsection{Fast Rates for Semi-Stochastic Sequences}

\begin{definition} We say that $(\matH_t)$ is a $(\kappa,\gamma)$-semi stochastic sequence if, for all $1 \le s \le t \le T$,
\begin{align*}
\sum_{i = s}^t \matH_t^\top \matH_t \succeq \kappa I - \gamma.
\end{align*}
\end{definition}

==> body/control_proofs.tex <==
%!TEX root = ../so_control_main.tex

\section{Proof of Control Bounds}
In this section, we demonstrate how our main guarantees for online learning - \Cref{thm:semions_memory} for the known sytem and \Cref{thm:semions_unknown} for the unknown system - imply bounds for non-stochastic control. Throughout, for simplicity, we assume $\radcomp,\radnat,\Rpinot \ge 1$. 

\subsection{Known System}
When the system is known (e.g. $\Ghat = \Gst$), \Cref{eq:recover_stuff} exactly recovers $\ypinothat = \ypinot,\upinothat = \upinot$. Therefore, our analysis considers the following regret benchmark:
\begin{align*}
\dfcreg_T(\Alg;\calM) := F_t(\matM_{t:t-h}\midypinot{t}) -  \inf_{M \in \calM} \sum_{t=1}^T f_t(\matM_t \midypinot{t})
\end{align*} 
To begin, we distill the arguments of \cite{simchowitz2020improper} into a black-box reduction from controller regret to the convex metric $\dfcreg_T(\Alg;\calM)$: 
\begin{proposition}\label{prop:DFC_reduction_known_system} Suppose that $\Alg$ is an adaptive DFC controller which uses $\ypinothat_t = \ypinot_t$ for all $t$, and let $\calM = \Mdfc(h,\radcomp)$. Then,
\begin{align*}
\Regret_T(\Alg;\Pi) \le \dfcreg_T(\Alg;\calM)  + 4 LT \radnat^2 \Rpinot^2 \radcomp^2 \left(\frac{\psicomp(h)}{\radcomp} + \frac{\psinot(h)}{\Rpinot}\right).
\end{align*}
\end{proposition}
The above is proved in \Cref{ssec:lem_dfc_reduction_known}. Next, we convert the assumptions from the control setting into bounds on the quantities which arise in \Cref{thm:semions_memory}. The following is proved in \Cref{sssec:lem:parameter_bounds_known}.
\begin{lemma}\label{lem:parameter_bounds_known} Let $\calM = \Mdfc(m,\radcomp)$, and let $\calC = \embedM(\calM)$, $\matY_t = \embedy(\ypinot_{t:t-h})$, $\matX_t = \sum_{i=0}^h \Gpinot^{[t-i]}\matY_t$. Then, 
\begin{enumerate}
\item $D = \diam(\calC) \le 2\radcomp \sqrt{h}$
\item $\radyc = \max_t\max_{z \in \calC}\|\matY_t z\| \le \radM\Rpinot$
\item $\radY = \max_t \|\matY_t\| \le \sqrt{h}\radnat$
\item $\radX \le \radG \radY$, $\radv = \radnat$, and $\Leff \le 2L \radnat \radcomp \Rpinot$. 
\end{enumerate}
\end{lemma}
We are now in a position to prove our main guarantee for controlling a known system:
\begin{proof}[Proof of \Cref{thm:known_control}]
\end{proof}
\subsection{Unknown System}
Next, let us turn to regret bounds for an unknown system. First, we will begin with an analysis assuming that we spend $N$ initial rounds in an estimation phase, which produces an estimate $\Ghat$ with suitable properties,  
\begin{condition}[Estimation Condition]\label{cond:estimation_setting} Consider the setting where $\Alg$ provides inputs 
\begin{align*}
\ualg_t = \uenalg_t + \uexalg_t, \quad \text{where } \uexalg_t = \begin{cases}  \uinit_t & t \in [N]\\
0 & t \in \{N+1,\dots,N+2h-1\}\\
\uen_t(\matM_t \midyhat{t}) & t \ge N+2h
\end{cases}.
\end{align*}
and where $\ypinothat_t$ is estimated in \Cref{eq:recover_stuff}, using an estimate $\Ghat$. We assume that $\Ghat^{[i]} = 0$ for all $i > 0$, that $\|\Gst - \Ghat\|_{\loneop} \le \epsG$, and that $\psinot(h) \Ru + 2\epsG \radM \radnat \le \radnat$. Lastly, we further assume that $\|\uinit_t\| \le \Ru$ for $t \le N$, 
\end{condition}
Since $\ypinothat_t$ are not exact, there is a feedback relationship between past inputs and future ones. Important, the above condition states that this feedback is not overwhelming, and that our parametrization is ``stable'' in the following sense:
\begin{lemma}[Stability]\label{lem:stability} Under \Cref{asm:estimation_setting}, we have
\begin{align*}
\|\ypinothat_t\| \le 2\radnat,  \quad \forall t \ge N+h.
\end{align*}
Moreover, for $t > N$, $\|\uexalg_t\| \le 2\radnat \radM$.
\end{lemma}
Next, we define a convex benchmark for regret which differs from the benchmark for the known system in two respects: (a) we consider time steps after $N + 2h$ (after the initial estimation phase) and (b), the benchmark considers controls based on the estimate $\ypinothat_t$ sequence:
\begin{align*}
\dfcreg_{T;T_0}(\Alg;\calM,\ypinothat) := \sum_{t=T_0}^T \Fcost_t(\matM_{t:t-h} \midyhat{t}) -  \inf_{M \in \calM} \sum_{t=T_0}^T \fcost_t(M \midypinot{t}), \quad T_0 = N+2h.
\end{align*}
The next step is to define an analogue of the reduction \Cref{prop:DFC_reduction_known_system} for unknown systems:
\begin{proposition}[DFC-Reduction Unknown]\label{prop:DFC_reduction_unknown} Set $T_0 = N+3h$, and let $N \ge 3h$, and suppose \Cref{asm:estimation_setting} holds. Moreover, let $\calM = \calM(h,\radM)$, where $\radM \ge \radcomp$. Then, 
\begin{align*}
\Regret_T(\Alg;\Pi) &\le \dfcreg_{T;N+2h}(\Alg;\calM,\ypinothat) + 8LN(\radnat + \Rpinot \radu)^2.\\
&\quad+ 11L\Rpinot^2 (\radM \radnat + \Ru)^2 \left(  \frac{\constpinot \psinot(h)}{\Rpinot} + \frac{\constpinot \psinot(h)}{\Rpinot}\right).
\end{align*}
\end{proposition}
So far, the above arguments are straightforward applications of those from \cite{simchowitz2020improper}. 
\paragraph{Accounting for Estimation Error in $\ypinothat_t$}


\subsubsection{Omitted Proofs}
\begin{lemma}\label{lem:input_error} Let $\Mapprox,\Mst \in \calM(M,\radM)$. Then,
\begin{align*}
\sum_{t=T_0}^T |f_t(\Mapprox \midyhat{t}) - f_t(\Mst \midypinot{t})| \le 4L\radGst^2\radM \radnat\sum_{t=T_0}^T \max_{i=0}^{h-1}\|\uex_t(\Mapprox \midyhat{t}) - \uex_t(\Mst \midypinot{t})\|_2
\end{align*}
\end{lemma}

\begin{lemma}\label{lem:y_est_sensitivity} For any parameter $\nu > 0$, we have the following inequality:
\begin{align*}
\sum_{t=T_0}^T |f_t(\Mapprox \midyhat{t}) - f_t(\Mst \midypinot{t})| &\le L \nu \sum_{t=T_0}^T \|\uexalg_{t} - \uex_{t}(\Mapprox \midyhat{t})\|_2^2\\
&\quad+ \constquad\cdot \frac{T\epsG^2}{\min\{\nu,1\}} + \consttrunc \cdot (T\psinot(h)+h),
\end{align*}
where $\constquad :=  20L\radGst^4\radnat^2\radM^4 $ and $\consttrunc := 4L \radGst^2 \radM  (2\radnat \radM + \Ru)^2$.
\end{lemma}


==> body/main_results.tex <==
%!TEX root = ../so_control_main.tex

\nipsminpt
\nipsminpt
\nipsminpt

\section{Main Results \label{sec:main}}
\nipsminpt
\nipsminpt
\paragraph{Policy Benchmark and Assumptions}
Our goal is be to have total cost which competes with stabilizing, linear controllers. Formally, a linear dynamical controller, or \emph{LDC}, is a is a linear dynamical system $(\Api,\Bpi,\Cpi,\Dpi) $, with internal state $\sopenpi_t \in \R^{\dimpi}$,  equipped with the internal dynamical equations $\sopenpi_{t+1} = \Api \sopenpi_t + \Bpi \yopenpi_t \quad \text{and} \quad \uopenpi_t := \Cpi \sopenpi_t + \Dpi \yopenpi_t$. 
We let $\Pildc$ denote the set of all LDC's $\pi$.  These policies include static fedback laws  $\uopenpi_t = K \yopenpi_t$, but are considerably more general due to the internal state. The \emph{closed loop} sequence $(\matypi_t,\matupi_t,\matxpi_t,\matspi_t)$ denotes the unique sequence consistent with  \Cref{eq:LDS_system}, the above internal dynamics, and the equalities $\uopenpi_t = \matu_t$, $\yopenpi_t = \maty_t$.\footnote{The sequence $(\yk_t,\uk_t)$ is a special case with $\Dpi = K$ and $\Cpi =0$.} We say consider \emph{stabilizing} $\pi$ meaning that, for all bounded disturbances sequences $\max_{t \ge 1} \|\matw_t\|,\|\mate_t\| <\infty$, it holds that $\max_{t \ge 1} \|\matypi_t\|,\|\matupi_t\| < \infty$. Since stabilizing policies enjoy geometric decay, our policy benchmark is pararametrized as follows:
\begin{definition}[Policy Benchmark]\label{defn:benchmark} Fix parameters $\rhocomp \in (0,1)$ and $\constcomp > 0$. Our regret benchmark competes LDC's $\pi \in \Pistar := \Pistab(\constcomp,\rhocomp)$, where we define
\iftoggle{nips}
{
	$\Pistab(c,\rho) := \{\pi \in \Pildc : (\|\Gpicl^{[i]}\|_{\op} \le c\rho^n, \forall n \ge 0\}$,
}
{
	\begin{align*}
\Pistab(c,\rho) := \{\pi \in \Pildc : \|\Gpicl^{[i]}\|_{\op} \le c\rho^n, \forall n \ge 0\},
\end{align*}
}
where the Markov operator $\Gpicl$ is formally defined in \Cref{defn:gpicl}. 
\end{definition}
 %When competing with other static LDCs, however the operator $\Gkpi$ takes a convenient closed form (\Cref{eq:conversion_static_feedback_to_static}).
%For any stabilizing $\pi \in \Pildc$, $\Gkpi$ is the Markov operator of a stable linear dynamical system, and thus lies in $\Pi(R,c,\rho) $ for some $R,c,\rho$. For simplicity, we choose $\radcomp \ge \Rk$, $\constcomp \ge \constk$, and $\rhocomp \ge \rhok$, so that the policy $\pi^K$ corresponding to $\ualg_t = K\yalg_t$ is in $\Pistar$. 
%Note that, while we assume the system is stabilized by a static $K$, we compete with arbitrary LDCs which have internal state.
Next, we turn to the necessary assumptions under which our bounds hold:
\begin{comment}
\begin{assumption}\label{asm:stab}For some $\constk > 0$ and $\rhok \in (0,1)$ and all $n \ge 0$, $\|\Gk^{[i]}\|_{\op} \le \constk\,\rhok^n$. %For simplicity, we assume that $\constk \le \constcomp,\rhok\le\rhocomp$.
\end{assumption}
\begin{assumption}\label{asm:bound}
We assume that $(\matw_t,\mate_t)$ are bounded such that, for all $t \ge 1$, $\|(\yk_t,\uk_t)\|_{2} \le \radnat$, where we recall that $(\yk_t,\uk_t)$ are interates under $\yalg_t = K\ualg_t$. For simplicity, we take $\matx_1 = 0$.
\end{assumption}
\Cref{asm:loss_reg} captures general smoothness and growth bounds for quadratic functions. \Cref{asm:stab} is analogous to ``strong stability'' \cite{cohen2018online}, and holds for some $\rhok \in (0,1),\constk > 0$ for any stabilizing $K$. Regarding \Cref{asm:bound}: since $K$ is stabilizing, any bounded sequence of disturbances will yield a uniform upper bound on $\|(\yk_t,\uk_t)\|_{2}$, and the assumption can be restated to depend directly on $\max_{t}\|\matw_t,\mate_t\|_2$.
%; following \citet{simchowitz2020improper}, we find it more natural to state our bound in terms of these quantities. 
Moreover, one may allow $\radnat$ to grow logarithmically in $T$ (e.g. $\radnat = \mathcal{O}(\log^{1/2} T)$ for subguassian noise), by inflating logarithmic factors in our bounds.
\end{comment}
%%In \Cref{app:general}, we describe generalizes to general decay functions, and stabilizing with static $K$.


Complete descriptions of \Cref{alg:nfc,alg:estimation_static} referenced above are detailed in \Cref{app:general}. The proof of the above theorems rests on generic policy regret bounds for the \semions{} algorithm, which are detailed in the following subsection. The proof of the above theorems is then completed in \Cref{sec:control_proofs_ful}, along with complete statements which specify the parameter choices \Cref{thm:drconsstat_known_granular,thm:drcons_unknown_specific}. In addition, \Cref{app:general} describes  generalizations which replace \emph{static} $K$ in the \drc{} algorithm with a dynamic nominal controller $\pinot$,
%\footnote{Note however that our \emph{benchmark} with the present, static $K$ variant is still all stabilizing controllers, not necessarily static.}, 
and \Cref{sec:control_proofs_ful} states and proves regret bounds for this more general algorithm as well. 
\nipsminpt
\nipsminpt
\nipsminpt
\nipsminpt
\subsection{Policy Regret for \semions\label{ssec:semi_ons_guarantees_known}}
\nipsminpt
\nipsminpt
Our main results for control derive from general-purpose policy regret bounds for the \semions{} algorithm. Specifically,  we consider the $\PolicyRegret$ benchmark \Cref{eq:pol_reg}, evaluated on losses of the form \iftoggle{nips}{$F_t(z_{t:t-h}) = \cost_t(\matv_t + \sum_{i=0}^h G^{[i]}\matY_{t-i}z_{t-i})$, and $f_t(z) = F_t(z,\dots,z) = \cost_t(\matv_ t + \matH_t z) $,}{
	\begin{align*}
	F_t(z_{t:t-h}) = \cost_t(\matv_t + \sum_{i=0}^h G^{[i]}\matY_{t-i}z_{t-i}), \quad f_t(z) = F_t(z,\dots,z) = \cost_t(\matv_ t + \matH_t z),
	\end{align*}
}where $\matH_t := \sum_{i=0}^h G^{[i]}\matY_{t-i}$. To address the known system case, we consider generic bounds on policy regret when running $\semions$ on losses $(f_t,\matH_t)$.
To address unknown systems, we bound the policy regret when $\semions$ with losses $(\fhat_t,\matHhat_t)$, where
\iftoggle{nips}{ $\fhat_t(z) := \cost_t(\matvhat_t + \matHhat_t z)$, and $\matHhat_t = \sum_{i=0}^h \Ghat^{[i]}\matY_{t-i}$.
}
{
\begin{align*}
 \fhat_t(z) := \cost_t(\matvhat_t + \matHhat_t z), \quad \text{ and } \matHhat_t = \sum_{i=0}^h \Ghat^{[i]}\matY_{t-i}.
\end{align*}
}
We assume the following bounds:

\begin{restatable}{definition}{defnPolPars}\label{defn:pol_reg_pars} Set $\diamz := \max\{\|z-z'\|:z,z' \in \calC\}$, $\radY := \max_{t} \|\matY_t\|_{\op}$, and  $\radyc := \max_{t}\max_{z \in \calC}\|\matY_t z\|$. Further take $\radv := \max_{t} \max\{\|\matv_t\|_2, \|\matvhat_t\|_2\}$ and we define $\radG := \max\{1,\|G\|_{\loneop},\|\Ghat\|_{\loneop}\}$, where $\|G\|_{\loneop} := \sum_{i \ge 0}\|G^{[i]}\|_{\op}$ Finally, we set $\radH = \radG \radY$, and define the the effective Lipschitz constant  $\Leff := L\max\{1,\radv + \radGst \radyc\}$. 
\end{restatable}
\iftoggle{nips}{}{Note that we let $\matz_{t},\matY_t$ be arbitrary even for $t \le 1$, provided the above bounds hold.}
In addition, our analysis hinges on $G$ having the following `invertibility' property: that  its smallest singular value, viewed as an operator on sequences $(u_{1},u_{2},\dots)$, is bounded below: 
\begin{definition}\label{defn:input_recov}  Let $G = (G^{[i]})_{i \ge 0}$ be a Markov operator. We define its \emph{invertibility-modulus} as
\iftoggle{nips}{
$\kappa(G) := 1 \wedge \inf_{(u_{0},u_{1},\dots)} \{\sum_{n \ge 0}\|\sum_{i=0}^n G^{[i]}u_{n-i}\|_2^2 : \sum_{t}\|u_t\|_2^2 = 1 \}$.
}
{
	\begin{align*}
\kappa(G) := 1 \wedge \inf_{(u_{0},u_{1},\dots)} \left\{\sum_{n \ge 0}\left\|\sum_{i=0}^n G^{[i]}\matu_{n-i}\right\|_2^2 : \sum_{t\ge 0}\|\matu_t\|_2^2 = 1 \right\}
\end{align*}
}
We also define its \emph{decay-function} $\psiG(n) := \sum_{i \ge n} \|G\|^{[i]}$, which is exponentially decay in the control setting.
\end{definition}
Our subsequent policy regret bounds will rely on $\kappa := \kappa(G) > 0$. Importantly, this assumption holds for our control setting (see \Cref{app:invertibility} for a proof):

Our subsequent analysis centers around the fact that, for $\kappa(G) > 0$, the covariance of the $\matH_t$ sequence dominates that of the $\matY_t$ sequence, up to lower order terms:


This implies roughly that the precondition dominates the $\matY$-convariance: $\Lambda_t \succsim  \lambda I + \sum_{s=1-h}^{t} \matY_{s}^{\top}\matY_{s}$ which is at the heart of the following regret bound. With this insight, we prove our first theorem, yielding logarithmic regret for $\kappa > 0$:

\begin{proof}[Proof Sketch] Since $f_t(z) = F_t(z,\dots,z) = \ell_t(\matv_t + \matH_t v)$, the preconditioner increments lie in a certain ``sweet spot'' $\Omega(1)\cdot \nabla f_t(\nabla f_t)^\top  \preceq  \matH_t^\top \matH \preceq \frac{1}{\alpha}\nablatwo f_t$ (\Cref{lem:ft_facts,lem:quad_lb}). This lets us to replicate the standard analysis of Online Newton Step \cite{hazan2007logarithmic} to bound $f$-regret (\Cref{thm:semions}).  From \Cref{lem:Ft_diff}, it remains to analyze the geometry-adaptive movement cost (\Cref{eq:geo_adaptive}). We use here that for $\kappa(G) > 0$,  invertibility of $G$ implies that $\Lambda_t$ roughly dominates the covariance of the $\matY_t$-sequence $\sum_{s=1-h}^t \matY_t^\top \matY_t$ (\Cref{prop:covariance_lb}). Thus, we can analyze \Cref{eq:geo_adaptive} as if $\Lambda_t$ were based on the $\matY_t$-geometry, which yields logarithmic geometry-aware movement by an application of the log-det potential lemma (\Cref{lem:log_potential}). The full proof is detailed in \Cref{sec:known}.
\end{proof}
%In particular, under \Cref{asm:stab}, we can take $h = 1+\frac{1}{1-\rho}\log(1 + C T)$, yielding a regret of  $\BigOhSt{\frac{1}{\alpha \kappa_0}\log^3 T},$, where $\BigOhSt{\cdot}$ hides polynomial dependence in other problem parameters.
%\end{theorem}
\nipsminpt
\nipsminpt
\nipsminpt
Lastly, we state the guarantee pertinent for \semions{} on approximate losses, bounding the policy regret on the $f_t,F_t$ sequence, but using updates from the estimates $\fhat_t$ defined above: 

%\begin{align}
%\PolRegplus_T(\nu;\zst) &:= \sum_{t=1}^T F_t(\matz_{t:t-h}) - f_t(\zst) + \nu\sum_{t=1}^T \|\matY_{t}(\matz_t - \zst)\|^2 \label{eq:polregplus_def_first}
%\end{align}
%We now \mscomment{\dots}

\begin{proof}[Proof Sketch] Using the geometry of the errors and AM-GM, the error introduced by the gradients of inexact $\fhat_t \approx f_t$ scales as  $\tau^{-1} T \epsG^2 + \tau \sum_{t=1}^T \|\matY_t(\matz_t - \zst)\|_2^2$, where $\tau$ is a free parameter, and where the second term measures distance between iterates $\matz_t$ and a comparator $\zst$ in $\matY_t$-geometry. Fortunately, our regret bound also contains a \emph{negative term} scaling as $- \sum_{t=1}^T \|\matX_t(\matz_t - \zst)\|_2^2$, which we use to offset the previous term. \iftoggle{nips}{}
{

}
By making $\tau$ small, we would like to show roughly that $\tau \sum_{t=1}^T \|\matY_t(\matz_t - \zst)\|_2^2 - \sum_{t=1}^T \|\matX_t(\matz_t - \zst)\|_2^2$ is non-positive. But this does not directly follow in the PSD-order comparison from \Cref{prop:covariance_lb}, because the vectors $\matz_t - \zst$ vary with $t$. Instead, we \emph{block} times $t$ into epochs of size roughly $\sqrt{T}$. We then argue that for large enough regularizer $\lambda \sim \sqrt{T}$, the iterates do not move too much within the blocks, allowing us to use \Cref{prop:covariance_lb}. The argument is quite careful, and a full proof is given in \Cref{sec:unknown}.
\end{proof}
\nipsminpt
\nipsminpt
\nipsminpt
In fact, the above technique yields a stronger version of the theorem, which also incorporates a \emph{negative term} in the regret scaling with  $\sum_{t=1}^T \|\matY_{t}(\matz_t - \zst)\|^2 $ (\Cref{thm:semions_unknown_clam}); this offset term is essential in obtaining fast rates for the control problem by accounting for the mismatch between $\matY_t = \embed(\yk_{t:t\shortminus m +1})$ based on the estimates of $\yk$, and the true $\yk_{t:t\shortminus m +1}$ (see \Cref{sssec:prop_redux_unknown}).  More generally, we remark that negative regret is in fact a cornerstone of the study of online learning with curvature (e.g., \citep{rakhlin2014online}). In addition, we prove a more general bound, \Cref{thm:unknown_granular}, which accomodates $\epsG^2 \ll \sqrt{T}$, showing a $(T\epsG)^{2/3}$ regret scaling for very small $\epsG$.


==> body/old_intution.tex <==

\paragraph{OCO with Memory (\ocom)} Following past work \cite{agarwal2019online,agarwal2019logarithmic,hazan2019nonstochastic,simchowitz2020improper},  our algorithm leverages a convex parametrization of control policies. This yields a reduction to the online convex optimization with memory framework (\ocom) of \citet{anava2015online}, facillitating low regret.  For simplicity, we illustrate this reduction for obtaining logarithmic regret for known system dynamics (\Cref{thm:known_control}). We shall let $z \in \R^d$ parameterize our control policies: at each $t$, \drcons{} selects control-input $\ualg_t$ according to policy $\matz_t$.\footnote{Specifically, $\matz_t$ encodes a mapping from past inputs and observations to current input $\ualg_t$; see \Cref{sec:prelim}.} The \ocom{} reduction then bounds $\Regret_T$ by roughly
\begin{align}\label{eq:pol_reg}
 \PolicyRegret_T := \sum_{t=1}^T F_t(\matz_{t},\matz_{t-1},\dots,\matz_{t-h}) - \inf_{z \in \calC} \sum_{t=1}^T f_t(z),
\end{align}
where the with-memory loss $F_t(\matz_{t:h})$ captures the cost at time $t$ of the algorithm incurred by selecting past policies $\matz_{t},\dots,\matz_{t-h}$ (truncating memory of the past to length $h$ steps), and where the unary loss $f_t(z) = F_t(z,\dots,z)$ capture the loss if the learner commited to the fixed policy parametrized by $z$ for all times.  We use the \drc{} parametrization \citep{simchowitz2020improper}, ensuring that $f_t$ are convex and determined by  the adversary's choices up to time $t$.
\iftoggle{nips}{}
{
	
}

Considering policy regret, rather than the standard $f\text{-regret}:=\sum_{t=1}^T f_t(\matz_{t}) - \inf_{z \in \calC} \sum_{t=1}^T f_t(z)$ is crucial for accounting for the so-called price of past mistakes. In particular, controlling policy regret is \emph{more challenging} than standard online learning because current actions influence future losses, via this memory. Nevertheless, prior work minimizes policy regret by running online learning procedures directly on the $f_t$ sequence - typically gradient descent updates $\matz_{t+1} \leftarrow \matz_t - \eta \nabla f_t(\matz_t)$. Moreover, the excess of policy regret over the $f$-regret is bounded by $ \text{($f$-regret)} +  \text{(movement cost)} $, where 
\iftoggle{nips}
{
$\text{ (movement cost) }  \approx \sum_{i=1}^h\sum_{t=1}^T\|\matz_t - \matz_{t-i}\|_2$
}
{
	\begin{align*}
 \,\, \text{ (movement cost) }  \approx \sum_{i=1}^h\sum_{t=1}^T\|\matz_t - \matz_{t-i}\|_2
\end{align*}
}
measures total movement of the iterates in the Euclidean norm. If the iterates move slowly enough that $\matz_{t} \approx \matz_{t-1} \approx \matz_{t:h}$, then  $F_t(\matz_{t:t-h}) \approx f_t(\matz_t)$, so policy regret tracks $f$-regret  \citep{anava2015online,even2009online,abbasi2014tracking}.
\nipsminpt
\nipsminpt
\nipsminpt
\paragraph{The perils of unpredictable curvature} 
%Fortunately, natural online learning procedures produce slow-moving iterates.  
Given any sequence of strongly convex losses $f_t$, online gradient descent with step sizes $\eta_t = \calO(1/t)$ produces $\calO(\log T)$ $f$-regret \citep{hazan2019introduction}. The uniform curvature assured by strong convexity enables this rapidly decaying step, which in turns ensures that the movement cost also scales as $\calO(h^2\log T)$, yielding logarithmic policy regret \citep{anava2015online}. For fully adversarial noise, however, $f_t$ might not be strongly convex, because fully adversarial noise may accumulate unevenly in different directions. In this case, there are second-order methods which can adapt the curvature of $f_t$ to attain logarithmic standard regret \cite{hazan2007logarithmic}. But these methods {fail} to enjoy logarithmic \emph{policy regret}, because the curvature induced by the $f_t$ sequence may not line up with the geometry required to achieve logarithmic movement cost \cite{foster2020logarithmic}. This problem is compounded by the fact that the relevant curvature of the problem is \emph{changing} as $f_t$ vary with time.

%In other words, simultansouly adapting to the $f_t$-geometry while mitigating sensitivity to past mistakes 


%Past work \citep{agarwal2019online,simchowitz2020improper} has demonstrated that the losses $f_t$ that arise in the control-to-policy-regret reduction are strongly convex, - thereby ensuring logarithmic regret -  provided the costs $\ell_t$ are strongly-convex, and the noise is stochastic-plus-adversarial with a non-degenerate stochastic component. 
%Due to the adversarial losses and partiall adversarial noise, these settings do not allow the learner to plan the optimal policy by learning a model of the dynamics. Rather, partially stochastic dyanmics let the learner forecast the \emph{geometry} of future losses: namely, uniform curvature in every direction. This is what enables the learner to choose conversative step sizes, and avoid movement cost. 

%Thus, low-regret online learning algorithms for truly non-stochastic noise may need to take aggressive steps in directions with less curvature. Thus, the key challenge in attain fast rates for non-stochastic control is \emph{adapting to unpredictable, time-varying problem geometry} \citep{foster2020logarithmic}.

%\mscomment{but if curvature changges, then there will be a big movement cost explain}
%and thus be penalized for mistakenly large  \emph{unforseen} changes in curvature via large (Euclidean) movement cost . 
%And while there are algorithms that attain logarithmic standard regret for generalizations of non-strongly convex losses (e.g. exp-concave losses), no such generalizations exist for policy regret, because there is no principled way to control movement cost. 
%This is true even if the losses are adversarial, and the noise has an adversarial component. Thus, stochastic noise does not make the future exactly `predictable'; rather, it ensures that

%The above suggests that stochastic noise helps not so much directly with forecasting, but with ensuring a consistent ``problem geometry''. \mscomment{meta-forecast about how agressively to update the control policy} Specifically, with stochastic noise, the learner ensures that past and future $f_t$ have similar curvature, whic... 
\nipsminpt
\nipsminpt
\nipsminpt
\paragraph{Adapting to changing geometry}
 In \Cref{sec:prelim},  we show that the with-memory losses in non-stochastic control  have a specific convolutional structure:  $\Fcost_t(z_{t:t-h}) := \loss_t(\matv_t + \sum_{i=0}^h G^{[i]}\,\matY_{t-i}z_{t-i} )$, where matrices $G^{[i]}$ are determined by the dynamical equations and fixed across $t$ , and time-varying $\matv_t$ and $\matY_t$ depend on disturbances up to time $t$. This structure allows our analysis to replace Euclidean movement cost with a geometry-adaptive analogue defined by $\matY_t$'s: 
\begin{align}
\text{ (geometry-adaptive movement cost) }  \approx \sum_{i=1}^h\sum_{t=1}^T\|\matY_t(\matz_t - \matz_{t-i})\|_2. \label{eq:geo_adaptive}
\end{align}
We stress that $\matY_t$ is not known to the learner before time $t$. Nevertheless,  we attain low policy regret via a simple variant of the Online Newton Step Algorithm (\ons{}\cite{hazan2007logarithmic}) that we call  Online Semi-Newton Step (\semions{}, \Cref{alg:semions}). \semions{} {adapts} to the $\matY_t$ geometry to \emph{enjoy logarithmic movement cost, while simultaneously achieving logarithmic $f$-regret}. This translates into logarithmic policy regret (\Cref{thm:semions_memory}), and thus logarithmic regret for our control problem (\Cref{thm:known_control}).


Unlike previous approaches, \semions{} is a grey-box optimization learning algorithm: it takes Newton-like steps $\matz_{t+1} \gets \matz_t  - \Lambda_t^{-1} \nabla f_t(\matz_t)$, where the preconditioner $\Lambda_t:= \lambda I + \sum_{s=1}^t\matH_t^\top \matH_t$ is constructed using the matrices $\matH_t := \sum_{i=0}^h G^{[i]}\,\matY_{t-i}$. The idea is that $\Lambda_t$ is essentially the ``largest'' preconditioner possible (in a PSD sense), subject to logarithmic $f$-regret (see also \Cref{rem:not_use_Hessian}). This desirable because larger $\Lambda_t$ means slower steps, slower moving iterates, and thus smaller movement cost.  Leveraging a special ``invertibility'' property that arises in the control setting (\Cref{defn:input_recov}), we show that each $\Lambda_t$ roughly dominates the covariance of the $\matY_t$-sequence - $\Lambda_t \succsim \sum_{s=1-h}^t \matY_t^\top \matY_t$ (\Cref{prop:covariance_lb}), despite being constructed from the $\matH_t$-sequence,. This is the key step in bounding movement cost.
%hinges on the fact that the $G^{[i]}$ matrices which arise in the control setting satisfy a certain `invertibility' condition (\Cref{defn:input_recov}).  
In contrast, standard Online Newton Step preconditioner based on rank-one gradient outer products \cite{hazan2007logarithmic}  may be too ``small'' (in a PSD sense) to achieve the same guarantee. See the proof sketch following \Cref{thm:semions_memory} for further proof details.

\nipsminpt
\nipsminpt
\nipsminpt
\paragraph{Sensitivity to error} For unknown dynamics, we cannot access the functions $f_t$ exactly, and instead run \semions{} with $\epsilon$-accurate approximations $\fhat_t$ based on estimated dynamics. The dominant term in the regret is no longer the iterate movement, but rather the sensitivity of the algorithm to $\epsilon$. For the $\sqrt{T}$ rate, we must show that \drcons{} has quadratic senstivity to $\epsilon$, incurring at most $T \epsilon^2$ extra regret for this error. Achieving  this quadratic sensitivity is ultimately somewhat involved but, a high level, the argument relies on the same key insights that facillitate the logarithmic regret for the known dynamics: we analyze sensitivity to error in the geometry introduced by the $\matY_t$ sequence, and relate this to the $\matH_t$-geometry induced by the algorithm. Further details are provided in the proof sketch following \Cref{thm:semions_unknown}.




==> body/online_newton.tex <==
%!TEX root = main.tex


\section{The Online Newton Step}
We use bold terms to denote terms either produced by the learner, or which correspond to terms produced by system dynamics 
Let us consider the online newton step algorithm, detailed below

\begin{comment}
\begin{algorithm}
\begin{algorithmic}[1]
    \State \textbf{parameters}: Learning rate
    $\eta>0$, regularization parameter $\veps>0$, convex constraint set $\cC$, matrix $\Gamma$
    \For{$t = 1,\dots,h$}
    \State{} Play $\matz_t = 0$ 
    \EndFor
    \State \textbf{initialize}: instance $\calA$ of $\semions(\lambda,\eta,\cC)$, with iterates $\matz_{s}^{\calA}$, and triples $(\ell_t^{\calA},\matv_t^{\calA},\matX_t^{\calA})$
    \For{$t=h+1,h+2,\dots$:}
    \State{} \textbf{play} iterate $\matz_{t} \leftarrow \matz_{t-h}^{\calA}$. 
    \State{} \textbf{recieve} function $F_t(z_t,\dots,z_{t-h}) = \loss_t\left(\matv_t+\sum_{i=0}^h G^{[i]} \matY_{t-i}z_{t-i}\right)$.
    \State{} \textbf{define} $\matvbar_t = \Gamma\matv_t$ and $\matXbar_t = \Gamma\matX_t$, $\lossbar_t(\cdot) = \loss_t(\Gamma^{\dagger}\cdot)$.
    \State{} \textbf{feed} $\calA$ the triple $(\ell_{t-h}^{\calA},\matv_{t-h}^{\calA},\matX_{t-h}^{\calA}) \leftarrow (\lossbar_t,\matvbar_t,\matXbar_t)$.
    \EndFor
  \end{algorithmic}
  \caption{Shaped Online Semi-Newton With Memory ($\shapeons(\lambda,\eta,\cC,\Gamma)$)}
  \label{alg:ohs}
\end{algorithm}
\end{comment}

\section{Preliminaries}
\begin{definition}
\end{definition}






